Axion dark matter search with a photonic bandgap cavity haloscope and dielectric tuning rod over 10.25-10.45 GHz

We report the development of a new widely tunable cavity and demonstrate its use in a search for dark matter axions. We achieve unloaded quality factors above $10^{5}$, roughly $25\times$ larger than a bare copper cavity at the same frequency, using concentric sapphire shells to reduce Ohmic losses on the cavity barrel. A rotating sapphire rod tunes our cavity mode over the $10.1-11.7$ GHz range, approximately $16\%$ of its resonant frequency. Using an amplified receiver chain, we demonstrate sensitivity to new axion parameter space by tuning the cavity over the $200$ MHz range between $10.25-10.45$ GHz (42.4 - 43.2, $\mu$eV) to constrain the axion-to-photon coupling to $|g_{a\gamma\gamma}|$ $\leq$ 1 $\times$ $10^{-12}$ ${GeV}^{-1}$. This cavity can scan its tuning range about $9$ times faster compared to a bare copper cavity when paired with a photon counting device, laying the groundwork for a definitive search for the QCD axion over $10.1-11.7$ GHz.

==> Amplitude_oscillations.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=\columnwidth]{Figures/Cavity_Broadening_PRL.pdf}
  \caption[Cavity Broadening]{Mechanical oscillations in our dilution refrigerator cause the tuning rod to oscillate inside the cavity volume. This causes an oscillation of the cavity transfer function. Any tone incident on the slope of this transfer function will acquire amplitude modulations as it moves up and down on the transfer function. These amplitude modulations can be picked up by a spectrum analyzer. The top plot is the cavity transfer function, the bottom left plot is the power spectrum of one tone near the $3$ dB point of the cavity and one is far off-resonance. The difference in the two spectrum is the bottom right plot, showing distinct features attributable to tuning rod oscillations, with the dominant tuning rod oscillation being $\approx 125$ Hz}
  \label{fig:Cavity Broadening}
\end{figure}
\FloatBarrier
\indent To quantify any cavity broadening induced by tuning rod oscillations with our beryllium copper fins when the cavity was cooled to milli-Kelvin temperatures we bounced a continuous wave tone off the cavity at two frequencies: one that lay on the slope of the cavity's reflection transfer function near its $3$ dB point and another that was far off-resonance. \\
\indent For the tone that lies on the cavity's transfer function, the tuning rod oscillations will induce amplitude modulations as the transfer function oscillates underneath the tone. These amplitude modulations can be picked up by a spectrum analyzer and seen in a power spectrum measurement. This plot can be seen in Figure \ref{fig:Cavity Broadening}. From the lower plots we can see that the $3$ dB tone has distinct sidebands from the tone that did not bounce off the cavity. These sidebands are symmetric, so our modulation is pure amplitude modulation as we would expect. The first of these sidebands are noticeable at $\approx 125$ Hz. This corresponds to the frequency of the rod oscillations inside the cavity volume, let's call this $f_{\te{rod}}$. This rod oscillation will modulate the cavity frequency as 
\begin{equation}
f_{\te{cav}}(t) = f_{0} + \Delta_{f} \sin({2\pi f_{\te{rod}}t})
\end{equation} 
where $\Delta_{f}$ is the size of the cavity deviation due to the rod and $f_{0}$ is the resonance of the mode if the rod were perfectly still. To estimate the size of this deviation, we need to know how the tone we sent interacts with the cavity. What is important is the instantaneous detuning of the tone from the cavity resonance which we have denoted as $f_{\te{cav}}(t)$. Let's call this detuning $\delta (t) = f_{\te{tone}} - f_{\te{cav}}(t) = \delta_{0} - \Delta_{f} \sin({2\pi f_{\te{rod}}t})$ where $\delta_{0} = f_{\te{tone}} - f_{0}$. 
To see how the transfer function changes due to this detuning we can Taylor expand the linear transfer function $|S11|$ around $\delta (t)$:
\begin{equation}
   |S11| (\delta_{0} - \Delta_{f})  = |S11|\bigg|_{\delta_{0}}+ \left.\frac{d|S11|}{d\delta}\right|_{\delta_{0}} \Delta_{f} + \mathcal{O}\big(\Delta_{f}^{2}\big)
\end{equation}
where the $\sin({2\pi f_{\te{rod}}t}))$ dependence has been omitted for simplicity. If our tone $f_{\text{tone}}$ is not near the resonance and $\Delta_{f}$ is assumed to be much smaller than the cavity bandwidth, then we can exclude non-linear terms to give us the much simpler relation
\begin{equation}
     |S11| (\delta_{0} - \Delta_{f})  = |S11|\bigg|_{\delta_{0}}+ \left.\frac{d|S11|}{d\delta}\right|_{\delta_{0}} \Delta_{f} 
\end{equation}
which we can rewrite as 
\begin{equation}
    \Delta_{f} = \f{\Delta_{\text{S11}}}{\left.\frac{d|S11|}{d\delta}\right|_{\delta_{0}} }
\end{equation}
where $\Delta_{\text{S11}} =  |S11| (\delta_{0} - \Delta_{f}) - |S11|\bigg|_{\delta_{0}}$. From this relation and Figure \ref{fig:Cavity Broadening} we can estimate the size of these deviations. From the lower right plot we can see this $125$ Hz sideband sits at around $-40$ dBc below the carrier frequency. This $40$ dB is a linear factor of $0.01$. Without the rod we expect the transfer function to reduce the carrier tone amplitude by $\approx 0.7$ from the top plot in Figure \ref{fig:Cavity Broadening}, so $\Delta_{S11} = 0.7\times 0.01 = 0.007$. The top plot also tells us the slope is $2.08\times 10^{-6} \ \text{Hz}^{-1}$, so the estimated deviations become
\begin{equation} \label{Cavity Broadening}
    \Delta_{f} = \f{0.007}{2.08\times 10^{-6} \ \text{Hz}^{-1}} \approx 3.36 \ \text{kHz}.
\end{equation}
This is less than the overcoupled cavity bandwidth on the order of $0.3$ MHz, so the assumption that these deviations are less than the cavity bandwidth (or the scale over which the transfer function slope changes significantly) remains self-consistent. \\
\indent However, this $3$ kHz broadening is close to the axion bandwidth of $10$ kHz at $10$ GHz, so if we wanted to improve the internal quality factor to approach the axion cavity linewidth this may become an issue. But for the cavity bandwidths seen in this thesis this does not constitute significant broadening. 


==> Supplementary_Material.tex <==
This document provides additional details pertaining to the experiment described in the main text. Namely, the full wiring diagram of the experimental setup in our dilution refrigerator, the temperature of the piezoelectric motor during a cooldown to prevent freezing on the motor gears, and a characterization of mechanically induced cavity mode broadening. 
\subsection{Piezo Heating During Cooldown}
\indent From the main body, we thermally isolate the piezoelectric motor from the dilution refrigerator during a cooldown to prevent freezing. Even a few degrees difference has shown to be sufficient.
\begin{figure}[htbp]
\centering
\includegraphics[width=\columnwidth]{Figures/Motor_Still_Temp_Comp_PRL.pdf}
 \caption[Motor Temperature During Cooldown]{Temperature of the piezoelectric motor during a cooldown compared to the still plate of the refrigerator, where the motor is heat sunk to. Even a few degrees of difference between the motor and the refrigerator has been sufficient to get consistent use of the motor.}
 \label{fig:Motor Temperatures}
\end{figure}
\FloatBarrier
\subsection{Fridge Diagram}
\begin{figure}[htbp]
\centering
\includegraphics[width=\columnwidth, height=0.6\textheight, keepaspectratio]{Figures/PRL_Fridge_Schematic_with_B.pdf}
  \caption[Fridge Schematic]{Experimental setup inside the dilution refrigerator. Cavity parameters are measured either in transmission or reflection with a common output line. The cavity sits in the center of the magnet bore (dashed box), with the magnet heat sunk to the $4$ K stage of the refrigerator. While a JPA was installed it was not used due to unstable gain with the magnet ramped. In its place the HEMT amplifier was the first stage amplifier.}
  \label{fig:fridge wiring}
\end{figure}
\FloatBarrier
\subsection{Cavity Broadening}
\input{Amplitude_oscillations}
